DSI++: Updating Transformer Memory with New Documents

Differentiable Search Indices (DSIs) encode a corpus of documents in model parameters and use the same model to answer user queries directly. Despite the strong performance of DSI models, deploying them in situations where the corpus changes over time is computationally expensive because reindexing the corpus requires re-training the model. In this work, we introduce DSI++, a continual learning challenge for DSI to incrementally index new documents while being able to answer queries related to both previously and newly indexed documents. Across different model scales and document identifier representations, we show that continual indexing of new documents leads to considerable forgetting of previously indexed documents. We also hypothesize and verify that the model experiences forgetting events during training, leading to unstable learning. To mitigate these issues, we investigate two approaches. The first focuses on modifying the training dynamics. Flatter minima implicitly alleviate forgetting, so we optimize for flatter loss basins and show that the model stably memorizes more documents ($+12\%$). Next, we introduce a generative memory to sample pseudo-queries for documents and supplement them during continual indexing to prevent forgetting for the retrieval task. Extensive experiments on novel continual indexing benchmarks based on Natural Questions (NQ) and MS MARCO demonstrate that our proposed solution mitigates forgetting significantly. Concretely, it improves the average Hits@10 by $+21.1\%$ over competitive baselines for NQ and requires $6$ times fewer model updates compared to re-training the DSI model for incrementally indexing five corpora in a sequence.

==> emnlp2023-latex/sections/09_reproducibility_statement.tex <==
\section*{Reproducibility Statement}
We introduce a novel benchmark constructed from the existing and publicly available Natural Questions (NQ) \citep{kwiatkowski2019natural} and MS MARCO \citep{nguyen2016ms} datasets. In our benchmark, we split the NQ and MS MARCO datasets into different subsets to enable the development of continual learning systems. We plan to release these splits as a standard benchmark for future works in this space. Further, in \S\ref{sec:sam} and \S\ref{sec:addn_impl_details}, we detail all hyper-parameters to enable the reproducibility of all our experiments.
